Quantum Atom Optics: Theory and Applications to Quantum Technology

This is a pre-publication version of a forthcoming book on quantum atom optics. It is written as a senior undergraduate to junior graduate level textbook, assuming knowledge of basic quantum mechanics, and covers the basic principles of neutral atom matter wave systems with an emphasis on quantum technology applications. The topics covered include: introduction to second quantization of many-body systems, Bose-Einstein condensation, the order parameter and Gross-Pitaevskii equation, spin dynamics of atoms, spinor Bose-Einstein condensates, atom diffraction, atomic interferometry beyond the standard limit, quantum simulation, squeezing and entanglement with atomic ensembles, quantum information with atomic ensembles. This book would suit students who wish to obtain the necessary skills for working with neutral atom many-body atomic systems, or could be used as a text for an undergraduate or graduate level course (exercises are included throughout). This is a near-final draft of the book, but inevitably errors may be present. If any errors are found, we welcome you to contact us and it will be corrected before publication. (TB: tim.byrnes[at]nyu.edu, EI: ebube[at]nyu.edu)

==> foreword.tex <==
\chapter*{Foreword}
\noindent  Having never written a book foreword beforeward, I did the logical thing and Googled “How to write a book foreword.” I found the following information: 1. Be honest. 2. Use your unique voice. 3. Discuss your connection to the story and authors. 4. Mimic the style of the book. 5. Sign off. From these tidbits of insight, it sounds more like I am conducting an hour-long radio show and not writing a foreword for a book. Nevertheless, I shall endeavor to address each point in turn. \\

\noindent  {\it 1. Be honest:} When my friends and colleagues Tim Byrnes and Ebubechukwu Ilo-Okeke asked me to write the foreword to {\it Quantum Atom Optics}, I was initially delighted because I have been an active research in this field for over thirty years and I have many tens of publications in the field. Hence, I was a bit flabbergasted when they sent me a draft of the book upon which perusing that I discovered that they had not cited a single paper written by me. Thus, my original draft of this foreword was, “Not too shabby book by what’s his face and colleague.” Since then I have calmed down a bit, but could not let that one slide. Aside from this unintentional slight, the book is actually very nice. I attributed not referencing my papers to the foolishness of youth and the fact that my papers were published before the authors were born. The field of quantum atom optics is hence quite mature by now, although I’m not dead yet, and such a book is timely and I can’t say enough nice things about the authors. The book is an exhaustive primer of a field that has a plethora of applications to a host of quantum technologies —-- particularly quantum information processing and quantum sensing. It would make a very nice supplementary book to any course on this topic. In truth the book is a compendium of just about everything that is known in quantum atom optics and as such it will be a much-used reference for many years. \\

\noindent  {\it 2. Use your unique voice:} As you can see from the above, my voice is so unique that I often have to translate my anonymous referee reports into Russian and then back into English in order to disguise my writing style. I can assure you that {\it Quantum Atom Optics} is a much better read than that. It is in fact very well written and delightfully organized in a clear and enticing fashion. Each chapter builds on the previous chapters such the book builds reaches a true crescendo at the end, much like Ravel’s orchestration of {\it Bolero}. \\

\noindent {\it 3. Discuss your connection to the story and authors:} As I mentioned above, apparently unbeknownst to the authors, I have been working in the field of quantum atom optics for much of my career, and this book does an excellent job of covering the field. I have been collaborating with Tim and Ebube on this topic for five years now and we have a series of papers together, which gives me a unique insight into the writing of their book. \\

\noindent  {\it 4. Mimic the style of the book:} Well I can’t use my unique voice and mimic the style of the book, now can I? The book was written by two sane and distinguished scientists. I’m more of an extinguished scientist myself. \\ 

\noindent {\it 5. Sign off:} \\

\noindent Good bye and good luck, \\


%\includegraphics[scale=1]{figures/jonsignature.jpg} \\

\noindent Jonathan P. Dowling \\

\noindent  13 October 2019\\
\noindent  St. George, Louisiana



\vspace{1cm}

\noindent {\it Authors' comment:  We made the unfortunate mistake of sending a preliminary version of the manuscript with incomplete referencing.  We hope the current version better captures the relevant literature.  Among the many new references added, Prof. Dowling's seminal paper \citep{dowling2003quantum}, where the much quoted term ``Second Quantum Revolution'' is now included.  This, along with several other brilliantly named papers (``Quantum Optical Metrology --- The Lowdown on High-N00N States''), will live on forever in the field.  Rest in peace Jon, you were an absolute inspiration and will be missed by us all. }


















\endinput

